Magnetic flux in the Sun emerges unaffected by supergranular-scale surface flows

Magnetic flux emergence from the convection zone into the photosphere and beyond is a critical component of the behaviour of large-scale solar magnetism. Flux rarely emerges amid field-free areas at the surface, but when it does, the interaction between magnetism and plasma flows can be reliably explored. Prior ensemble studies identified weak flows forming near emergence locations, but the low signal-to-noise required averaging over the entire dataset, erasing information about variation across the sample. Here, we apply deep learning to achieve improved signal-to-noise, enabling a case-by-case study. We find that these associated flows are dissimilar across instances of emergence and also occur frequently in the quiet convective background. Our analysis suggests diminished influence of supergranular-scale convective flows and magnetic buoyancy on flux rise. Consistent with numerical evidence, we speculate that small-scale surface turbulence and / or deep-convective processes play an outsize role in driving flux emergence.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
